Notes on Using Control Variates for Estimation with Reversible MCMC Samplers

A general methodology is presented for the construction and effective use of control variates for reversible MCMC samplers. The values of the coefficients of the optimal linear combination of the control variates are computed, and adaptive, consistent MCMC estimators are derived for these optimal coefficients. All methodological and asymptotic arguments are rigorously justified. Numerous MCMC simulation examples from Bayesian inference applications demonstrate that the resulting variance reduction can be quite dramatic.

==> PS/MHPoisson.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Usage: -To include a Figure with a caption, insert the TWO following lines
%        in your Latex file:
% \input{This_file_name} 
% \dessin{The_caption}{The_label}
%         -To include just a picture, insert the lines 
%         between \fbox{\begin{picture}...  and \end{picture}} below 
%          
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \long\def\Checksifdef#1#2#3{%
\expandafter\ifx\csname #1\endcsname\relax#2\else#3\fi}
\Checksifdef{Figdir}{\gdef\Figdir{}}{}
\def\dessin#1#2{
\begin{figure}[hbtp]
\begin{center}
%If you prefer cm use the following two lines
%\setlength{\unitlength}{1mm}
%\fbox{\begin{picture}(850.50,601.02)
\fbox{\begin{picture}(300.00,212.00)
% if you want to use epsfig uncomment the following line 
% and comment the special line 
%\epsfig{file=\Figdir MHPoisson.eps,width=300.00pt,height=212.00pt}
\special{psfile=\Figdir MHPoisson.eps hscale=100.00 vscale=100.00}
\end{picture}}
\end{center}
\caption{\label{#2}#1}
\end{figure}}


==> PS/binary_probit.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Usage: -To include a Figure with a caption, insert the TWO following lines
%        in your Latex file:
% \input{This_file_name} 
% \dessin{The_caption}{The_label}
%         -To include just a picture, insert the lines 
%         between \fbox{\begin{picture}...  and \end{picture}} below 
%          
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \long\def\Checksifdef#1#2#3{%
\expandafter\ifx\csname #1\endcsname\relax#2\else#3\fi}
\Checksifdef{Figdir}{\gdef\Figdir{}}{}
\def\dessin#1#2{
\begin{figure}[hbtp]
\begin{center}
%If you prefer cm use the following two lines
%\setlength{\unitlength}{1mm}
%\fbox{\begin{picture}(850.50,601.02)
\fbox{\begin{picture}(300.00,212.00)
% if you want to use epsfig uncomment the following line 
% and comment the special line 
%\epsfig{file=\Figdir binary_probit.eps,width=300.00pt,height=212.00pt}
\special{psfile=\Figdir binary_probit.eps hscale=100.00 vscale=100.00}
\end{picture}}
\end{center}
\caption{\label{#2}#1}
\end{figure}}


==> PS/binary_probit_alt.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Usage: -To include a Figure with a caption, insert the TWO following lines
%        in your Latex file:
% \input{This_file_name} 
% \dessin{The_caption}{The_label}
%         -To include just a picture, insert the lines 
%         between \fbox{\begin{picture}...  and \end{picture}} below 
%          
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \long\def\Checksifdef#1#2#3{%
\expandafter\ifx\csname #1\endcsname\relax#2\else#3\fi}
\Checksifdef{Figdir}{\gdef\Figdir{}}{}
\def\dessin#1#2{
\begin{figure}[hbtp]
\begin{center}
%If you prefer cm use the following two lines
%\setlength{\unitlength}{1mm}
%\fbox{\begin{picture}(850.50,601.02)
\fbox{\begin{picture}(300.00,212.00)
% if you want to use epsfig uncomment the following line 
% and comment the special line 
%\epsfig{file=\Figdir binary_probit_alt.eps,width=300.00pt,height=212.00pt}
\special{psfile=\Figdir binary_probit_alt.eps hscale=100.00 vscale=100.00}
\end{picture}}
\end{center}
\caption{\label{#2}#1}
\end{figure}}


==> PS/gibbsG.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Usage: -To include a Figure with a caption, insert the TWO following lines
%        in your Latex file:
% \input{This_file_name} 
% \dessin{The_caption}{The_label}
%         -To include just a picture, insert the lines 
%         between \fbox{\begin{picture}...  and \end{picture}} below 
%          
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \long\def\Checksifdef#1#2#3{%
\expandafter\ifx\csname #1\endcsname\relax#2\else#3\fi}
\Checksifdef{Figdir}{\gdef\Figdir{}}{}
\def\dessin#1#2{
\begin{figure}[hbtp]
\begin{center}
%If you prefer cm use the following two lines
%\setlength{\unitlength}{1mm}
%\fbox{\begin{picture}(850.50,601.02)
\fbox{\begin{picture}(300.00,212.00)
% if you want to use epsfig uncomment the following line 
% and comment the special line 
%\epsfig{file=\Figdir gibbsG.eps,width=300.00pt,height=212.00pt}
\special{psfile=\Figdir gibbsG.eps hscale=100.00 vscale=100.00}
\end{picture}}
\end{center}
\caption{\label{#2}#1}
\end{figure}}


==> PS/gibbsG2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Usage: -To include a Figure with a caption, insert the TWO following lines
%        in your Latex file:
% \input{This_file_name} 
% \dessin{The_caption}{The_label}
%         -To include just a picture, insert the lines 
%         between \fbox{\begin{picture}...  and \end{picture}} below 
%          
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \long\def\Checksifdef#1#2#3{%
\expandafter\ifx\csname #1\endcsname\relax#2\else#3\fi}
\Checksifdef{Figdir}{\gdef\Figdir{}}{}
\def\dessin#1#2{
\begin{figure}[hbtp]
\begin{center}
%If you prefer cm use the following two lines
%\setlength{\unitlength}{1mm}
%\fbox{\begin{picture}(850.50,601.02)
\fbox{\begin{picture}(300.00,212.00)
% if you want to use epsfig uncomment the following line 
% and comment the special line 
%\epsfig{file=\Figdir gibbsG2.eps,width=300.00pt,height=212.00pt}
\special{psfile=\Figdir gibbsG2.eps hscale=100.00 vscale=100.00}
\end{picture}}
\end{center}
\caption{\label{#2}#1}
\end{figure}}


==> PS/gibbsG3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Usage: -To include a Figure with a caption, insert the TWO following lines
%        in your Latex file:
% \input{This_file_name} 
% \dessin{The_caption}{The_label}
%         -To include just a picture, insert the lines 
%         between \fbox{\begin{picture}...  and \end{picture}} below 
%          
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \long\def\Checksifdef#1#2#3{%
\expandafter\ifx\csname #1\endcsname\relax#2\else#3\fi}
\Checksifdef{Figdir}{\gdef\Figdir{}}{}
\def\dessin#1#2{
\begin{figure}[hbtp]
\begin{center}
%If you prefer cm use the following two lines
%\setlength{\unitlength}{1mm}
%\fbox{\begin{picture}(850.50,601.02)
\fbox{\begin{picture}(300.00,212.00)
% if you want to use epsfig uncomment the following line 
% and comment the special line 
%\epsfig{file=\Figdir gibbsG3.eps,width=300.00pt,height=212.00pt}
\special{psfile=\Figdir gibbsG3.eps hscale=100.00 vscale=100.00}
\end{picture}}
\end{center}
\caption{\label{#2}#1}
\end{figure}}


==> PS/gibbsG5.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Usage: -To include a Figure with a caption, insert the TWO following lines
%        in your Latex file:
% \input{This_file_name} 
% \dessin{The_caption}{The_label}
%         -To include just a picture, insert the lines 
%         between \fbox{\begin{picture}...  and \end{picture}} below 
%          
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 \long\def\Checksifdef#1#2#3{%
\expandafter\ifx\csname #1\endcsname\relax#2\else#3\fi}
\Checksifdef{Figdir}{\gdef\Figdir{}}{}
\def\dessin#1#2{
\begin{figure}[hbtp]
\begin{center}
%If you prefer cm use the following two lines
%\setlength{\unitlength}{1mm}
%\fbox{\begin{picture}(850.50,601.02)
\fbox{\begin{picture}(300.00,212.00)
% if you want to use epsfig uncomment the following line 
% and comment the special line 
%\epsfig{file=\Figdir gibbsG5.eps,width=300.00pt,height=212.00pt}
\special{psfile=\Figdir gibbsG5.eps hscale=100.00 vscale=100.00}
\end{picture}}
\end{center}
\caption{\label{#2}#1}
\end{figure}}

